Decoupling Adaptive Control in TeaStore

The Adaptable TeaStore specification provides a microservice-based case study for implementing self-adaptation through a control loop. We argue that implementations of this specification should be informed by key properties of self-adaptation: system-wide consistency (coordinated adaptations across replicas), planning (executing an adaptation until appropriate conditions are met), and modularity (clean integration of adaptation logic). In this implementation discussion paper, we examine how software architectural methods, the cloud-native Operator pattern, and legacy programming language techniques can decouple self-adaptive control logic from the TeaStore application. We analyze the trade-offs that these different approaches make between fine-grained expressive adaptation and system-wide control, and highlight when reuse of adaptation strategies is most effective. Our analysis suggests that these approaches are not mutually exclusive but can be combined into a multi-tiered architecture for self-adaptive microservices.

==> eptcsdata.tex <==
\providecommand{\firstpage}{40}
\providecommand{\publicationstatus}{G. De Palma and S. Giallorenzo (Eds.):\\
First Workshop on Adaptable Cloud Architectures\\
EPTCS 438, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.438.3}{10.4204/EPTCS.438.3}}
\pdfoutput=1
\usepackage{ifthen}
\providecommand{\eptcs}{{\sl Electronic Proceedings in Theoretical Computer Science}}
\providecommand{\opa}{, Open Publishing Association}
\providecommand{\finishreference}[6]{#1 #2#3, pp. #4--#5, \doi{10.4204/EPTCS.#2.#6}}
\providecommand{\thisvolume}[2][\eptcs]{%
 \ifthenelse{\equal{#2}{9}}{\finishreference{#1}{438}{\opa}{1}{14}{1}}{%
 this volume of #1\opa}}

